RIDS : Real-time Intrusion Detection System for WPA3 enabled Enterprise Networks

With the advent of new IEEE 802.11ax (WiFi 6) devices, enabling security is a priority. Since previous versions were found to have security vulnerabilities, to fix the most common security flaws, the WiFi Protected Access 3 (WPA3) got introduced. Although WPA3 is an improvement over its predecessor in terms of security, recently it was found that WPA3 has a few security vulnerabilities as well. In this paper, we have mentioned the previously known vulnerabilities in WPA3 and WPA2. In addition to that, we have created our own dataset based on WPA3 attacks (Section III). We have proposed a two-stage solution for the detection of an intrusion in the network. The two-stage approach will help ease computational processing burden of an AP and WLAN Controller. First, AP will perform a lightweight simple operation for some duration (say 500ms) at certain time interval. Upon discovering any abnormality in the flow of traffic an ML-based solution at the controller will detect the type of attack. Our approach is to utilize resources on AP as well as the back-end controller with certain level of optimization. We have achieved over 99% accuracy in attack detection using an ML-based solution. We have also publicly provided our code and dataset for the open-source research community, so that it can contribute for future research work.

==> rough.tex <==
% \section{Problem Statement}
% Wifi devices have evolved in terms of performance, resource management, and sophistication. Still, it's not enough to run any machine learning model over it. Due to the limitation of computational power and constrained resources. The backend controller system is also not enough to check each and every packet for attack analysis as it will overburden the system. The challenge is to maintain the resource utilization balance for an AP and the backend controller.

% \section{Proposed Solution}
% As mentioned in the problem statement, the proposed solution should work intelligently with respect to performance and resource utilization. In this paper, the solution proposed is based on two stages. First, we deploy an Intrusion Detection System (IDS)  on the AP side for verifying the packets based on a defined set of rules. This would help the backend controller from getting overwhelmed with packet analysis. Once IDS detects some intrusion or malicious activity. It will trigger the backend controller to start looking into the packet analysis for an attack. The second, stage consists of an ML-based model for packet analysis and generating alerts based on the analysis. ML-model can be deployed at the controller. This would help the detection of malicious users or activity. 

% \section{Attacks on WPA3}
% \label{attacks}

% Following attacks are being focused for the purpose of analysis. 

% % write about attacks here

% \subsection{De-authentication}
% The attack is possible in WPA2 and WPA3 as well. An attacker can force the STA to disconnect from AP using a de-authentication attack. WPA3 refrains attackers from spoofing the de-authentication frame once a 4-way handshake is completed, due to management frame protection (MFP). Although an attacker can still de-auth the STA by sending multiple de-authentication frames right after the association request from an STA to an AP. Thus results in creating an ambiguity for the STA to process succeeding packets from the AP. This will result in STA sending a de-authentication packet to the AP. Finally, the STA will be disconnected from establishing any connection to the AP.


% % \subsection{WPA3 Transient Mode}
% % Wifi devices are supposed to be backward compatible. This allows users with the previous version of devices to connect with the latest APs. The transition state is vulnerable to attacks. An attacker can configure hostapd 2.9 in such a way that it can transmit beacons at a higher rate, advertising a WPA2 connection for legitimate AP.  This will allow a victim device to connect to an AP with a WPA2 connection instead of a WPA3. The victim while the exchange of the third message of the handshake between STA and an AP. When AP will realize the STA is connecting using a WPA2 connection, will allow the STA to establish the connection using a WPA2 connection. This would expose the AP to WPA2 attacks.


% \subsection{Rogue AP}
% This attack involves configuring a fake AP using hostapd. Once a fake AP is created, an attacker can launch the AP with the same name, bssid as a legitimate AP, and broadcast at a lower beacon interval. This will let the STA trust the rogue AP and try to connect with it. In the case of the WPA3 AP, STA can be spoofed to connect with the WPA2 connection through our rogue AP. By lowering the beacon interval rogue AP can broadcast a WPA2 connection instead of WPA3. This will make STA connect using WPA2 authentication, STA will later acknowledge in message 3 of the 4-way handshake that AP connects using WPA3 authentication. This will result in denial of service for the STA, as it would detect the connection is based on WPA3 instead of WPA2.


% % \subsection{Evil Twin}
% % The attack is based on creating a fake AP. Just like we did in rogue AP. This time attacker tries to disconnect the STA from legitimate AP and connect to Evil Twin AP (ETAP). This will work in a scenario of open AP present in public places. If the AP is password protected and runs on the WPA2 authentication protocol then an attacker can run an offline dictionary attack on the AP. Once the password is discovered, an attacker can create ETAP entirely the same as legitimate AP.  This would result in a man-in-the-middle attack, flooding the network with garbage data, or even denial of service.


% \subsection{Beacon Flooding}
% The attack is simple and doesn’t require any intervention between STA and an AP. The beacon frames are not protected. An attacker can easily exploit them by flooding multiple beacon frames compared to a genuine AP. Sending multiple probe responses would increase the computation time for the STA to find the legitimate AP. If the probe responses are similar to an AP, then this would end up in denial of service to the STA. Since STA would try to connect to an SSID of a similar kind.


% \section{Detection of attacks}
% The initial detection model is based on traffic analysis of certain frames. As APs are resource-constrained and have limited capabilities in terms of performing intense computation. We propose a lightweight solution that is easy to implement and effective in case of early detection. The mechanism is primarily based on the following frames:
% \begin{enumerate}
%     \item Beacon Frame
%     \item Authentication Frame
%     \item De-authentication Frame
%     \item Association Frame
%     \item Dis-association Frame
%     \item EAPOL Frame
% \end{enumerate}

% The system will keep track of the above-mentioned frames in the traffic flowing through an AP. Then for a time quantum (say 10 seconds), AP will monitor the flow of traffic and keep a count of the above-mentioned frames. If for any instance number of frames exceeds 16 frames/seconds. Then we can assume suspicious behavior in the network traffic. For an attack to be successful an attacker would send packets at a higher rate. Similarly, a higher packet rate would signify that an attack is underway. 

% Once the IDS raises suspicion of an attack then our ML-based solution will analyze each packet and detect if an attack is going on or not. 



% \section{Detecting with Machine Learning}

% We used the AWID-3 Dataset which is collection of pcap files of various attacks performed on WPA-3. AWID-3 has been constructed from multiple attack sessions with a total of 254 attributes. The collection is based on traces of normal and intrusion attacks on an 802.11ax wifi network. The attacks considered in this research are De-authentication, Rogue AP, Beacon Flooding attacks. The dataset has pcap files that contain the packets transmitted in the network while the attacks were being performed. These packets can be analysed using a deterministic algorithm (as shown in Section \ref{attacks}) to detect the attacks. However, using ML we might be able to find a correlation between the attributes to detect the attacks. We used this data to train a few ML classifiers. We tested three different classifiers: 

% \begin{enumerate}
%     \item Logistic Regression
%     \item Decision Tree
%     \item Random Forest
% \end{enumerate}

% \subsection{Results}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{accuracy.eps}
%     \caption{Accuracy by Classifiers}
%     \label{fig:accuracy}
% \end{figure}

% As shown in Fig. \ref{fig:accuracy}, the accuracy of Decision Tree (98.68\%) and Random Forest (99.98\%) are comparable. We need to remember that the correct evaluation of a classifiers cannot be done just by comparing the accuracy. So we tested the classifier with multiple attack vectors and computed the confusion matrix for each classifier. As seen in the confusion matrices (Fig. \ref{fig:dt_cm}, \ref{fig:rf_cm}), Random Forest Classifier has the least number of false positives. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{dtree_cm_new.eps}
%     \caption{Confusion Matrix for Decision Tree}
%     \label{fig:dt_cm}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{rf_cm_new.eps}
%     \caption{Confusion Matrix for Random Forest}
%     \label{fig:rf_cm}
% \end{figure}

% Random Forest Classifier, as evident from Table \ref{table:fpr_tpr} has a really low false positive rate. We decided to choose Random Forest Classifier to predict the occurrence of an attack in real-time. Once our system rings an alert then the Classifier can start analysing packets and detect if the network has been attacked. This mix of algorithms (Non-ML Alert Phase and ML based Attack Detection) is useful for a network with very high bandwidth and multiple APs such that monitoring the network centrally for vulnerabilities is not feasible. In the next Section we propose a complete Attack Detection System for an enterprise scenario. With such a low false positive rate, Random Forest Classifier can precisely detect if the network is being attacked upon being triggered by the Alert Phase algorithm. 

% \begin{table}[h]
% \centering
% \caption{Comparison of FPR and TPR of Classifiers}
% \label{table:fpr_tpr}
% \begin{tabular}{|l|l|l|}
% \hline
% Metric & Decision Tree & Random Forest \\ \hline \hline
% FPR    & 0.0134        & 0.00068    \\ \hline
% TPR    & 0.9866    & 0.99932     \\ \hline
% \end{tabular}
% \end{table}




% \section{Experimental Setup}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{setup.png}
%     \caption{Experimental Setup}
%     \label{fig:setup}
% \end{figure}

% We created our dataset using different devices as shown in \ref{fig:setup}. For WPA3 enabled access point we used the Linksys E8450 device and for the WPA3 wifi adapter, D-link DWA-X1850 was used. One Alfa AWUS036NHA adapter (Atheros AR9271 chipset) was used for monitoring the channel and injecting packets for the purpose of performing attacks. Netgear A6210 device is used for monitoring traffic between AP and STAs. Netgear device was connected to a desktop running Ubuntu 20.04. For STAs we have used a Samsung A7 tablet, MacBook Air, and an HP laptop running windows 10 using a D-link adapter supporting WPA3. 

% The Linksys AP, we used supports 802.11ax, running in WPA3 mode on a 2.4 GHz frequency. All our attacks are performed on 2.4 GHz frequency only. The 5GHz frequency was also working but no attacks were performed on the 5GHz frequency. The Netgear A6210 adapter was used for the purpose of capturing packets works on dual-band. Figure x is just a representation of our setup for testing and collecting data. 


